Adaptive View Planning for Aerial 3D Reconstruction

With the proliferation of small aerial vehicles, acquiring close up aerial imagery for high quality reconstruction of complex scenes is gaining importance. We present an adaptive view planning method to collect such images in an automated fashion. We start by sampling a small set of views to build a coarse proxy to the scene. We then present (i)~a method that builds a view manifold for view selection, and (ii) an algorithm to select a sparse set of views. The vehicle then visits these viewpoints to cover the scene, and the procedure is repeated until reconstruction quality converges or a desired level of quality is achieved. The view manifold provides an effective efficiency/quality compromise between using the entire 6 degree of freedom pose space and using a single view hemisphere to select the views. Our results show that, in contrast to existing "explore and exploit" methods which collect only two sets of views, reconstruction quality can be drastically improved by adding a third set. They also indicate that three rounds of data collection is sufficient even for very complex scenes. We compare our algorithm to existing methods in three challenging scenes. We require each algorithm to select the same number of views. Our algorithm generates views which produce the least reconstruction error.

==> notations.tex <==
\section{Notations and Definition}
In this section, we formalize the view selection problem and present our notation. 
%We formulated the problem and present our notation in this section. 
Given a triangular mesh $\mathcal{M} = \{\mathcal{F}, \mathcal{V}\}$ built on a point clouds $\mathcal{G} = \{g_1,g_2,...,g_G\}$ with mesh vertices $\mathcal{V} = \{v_1,v_2,...,v_V\}$ and a set of faces $\mathcal{F} = \{f_1,f_2,...,f_F\}$, $f_i \in \mathcal{V} \times \mathcal{V} \times \mathcal{V}$, we would like to plan a trajectory with a minimum set of views $C = \{c_1,c_2,...,c_C\}$, $c_i \in \mathbb{R}^6$ that covers $\mathcal{F}$ with good quality, where the quality measure is defined in Section~\ref{sec:lqr}. 
Here, a camera view $c$ consists of 6 degree-of-freedom with $P_c\in \mathbb{R}^3$ for position and $R_c \in \mathbb{R}^3$ for rotation. 
For each face of the mesh $f \in \mathcal{M}$, we define $N_f$ and $N_v$  as the normal vector of the face $f$ and vertex $v$ respectively. We also define the center of the face as $P_f$.

\subsection{Visibility Cone Model}
In order to define the coverage of a scene, we first need to model the visibility of a face so that we can reason for the coverage of the scene.  

\begin{figure}
\centering
	\includegraphics[width=0.4\textwidth]{viscone.jpg}
	\caption{Visibility cone of a triangular mesh: the visibility cone infers the region of possible good views for the triangular mesh.}
	\label{fig:viscone}
\end{figure}

We model the visibility of each face of the mesh as a right circular cone denoted as $Cone(f)$ shown in Fig~\ref{fig:viscone}. If a view $c$ is within the visibility cone $Cone(f)$, the face $f$ is visible from the view $c$.
Because the scene is not fully known, we build the cone based on the existing views and infer the visible region with this model. 
Therefore, the cone apex angle denoted as $\Theta(f)$ is
\begin{equation}
\Theta(f) = \max_{c_i,c_j \in C_{init}} \angle(\overline{P_fc_i},\overline{P_fc_j}) \cdot I(f)
\end{equation}
where $I(f)$ is an indicator function. $I(f) = 1$ if and only if $c_i,c_j$ construct the face $f$. $C_{init}$ is the initial set of views that construct the scene. 
%For each triangular mesh, we define a camera view $p$ to be visible to the triangular mesh when the view contains a 2D feature that projects to 3D on the triangular mesh. 
$\Theta(f)$ is defined as the $\textit{visibility angle}$ of the face $f$. The cone axis is set to the face normal $N_f$.

The coverage of the scene is defined such that for each face $f \in \mathcal{F}$, there are at least two views $\{c_i,c_j\} \in Cone(f)$ within the visibility cone. The reconstruction quality is then defined as the angle between the camera pair $\{c_i,c_j\}$ with the face center $P_f$. In practice, high reconstruction quality requires not only the angular constraint but also the number of visible cameras. In Section~\ref{sec:lqr}, we incorporate these criteria to measure region quality.

However, the initial estimated mesh may contain bad faces that do not represent the true surface. Therefore, we provide an adaptive method that improves those faces iteratively. 

\subsection{Reconstruction Quality}\label{sec:lqr}
Low reconstruction quality regions are generally the regions that do not contain accurate points to be triangulated. Visually, the mesh or texture representation captures a much distorted geometry compared to reality. Those low quality regions are either occluded or low texture regions that cannot receive sufficient good views.  
For a complex scene, occluded and low-texture regions are hard to reconstruct without region-specific view planning. Therefore, we identify those regions in our model and plan the views only for the low quality region for refinement. It is much more efficient than planning the views for the entire scene. 

The reconstruction quality is mainly effected by three factors: the parallax between a pair of views, the distance between the target to the views, and the number of views that are visible to the region. 
Generally speaking, high parallax results in accurate triangulation while being hard to find feature correspondences. For views with significant distance variations to the target, the difference between resolution can pose difficulties to both sparse and dense reconstruction~\cite{zheng2014patchmatch}. However, only two views are not sufficient. During the feature matching process, additional detected features are used as validation process to ensure the detection accuracy. Therefore, more views can increase the number of correctly matched features per region. Thus, we define the quality $Q(f)$ of each face $f$ in the mesh as follows. 
\begin{equation}
	Q(f) = \frac{\sin{\Theta(f)}}{d^2}
\end{equation}
where $\Theta(f) = \max_{s_i,s_j \in \kappa(f)} (\angle(\overline{s_if_c},\overline{s_jf_c}))$ and $\kappa(f) = Vis(f) \bigcap J$ is a set of views that are visible to face $f$. 
%Essentially, the quality measure $Q(f)$ is the average number of visible cameras per face area weighted by the visibility angle. 
